Shelving it rather than Ditching it: Dynamically Debloating DEX and Native Methods of Android Applications without APK Modification

Today's Android developers tend to include numerous features to accommodate diverse user requirements, which inevitably leads to bloated apps. Yet more often than not, only a fraction of these features are frequently utilized by users, thus a bloated app costs dearly in potential vulnerabilities, expanded attack surfaces, and additional resource consumption. Especially in the event of severe security incidents, users have the need to block vulnerable functionalities immediately. Existing works have proposed various code debloating approaches for identifying and removing features of executable components. However, they typically involve static modification of files (and, for Android apps, repackaging of APKs, too), which lacks user convenience let alone undermining the security model of Android due to the compromising of public key verification and code integrity checks. This paper introduces 3DNDroid, a Dynamic Debloating approach targeting both DEX and Native methods in AnDroid apps. Using an unprivileged management app in tandem with a customized Android OS, 3DNDroid dynamically reduces unnecessary code loading during app execution based on a pre-generated debloating schema from static or dynamic analyses. It intercepts invocations of debloated bytecode methods to prevent their interpretation, compilation, and execution, while zero-filling memory spaces of debloated native methods during code loading. Evaluation demonstrates 3DNDroid's ability to debloat 187 DEX methods and 30 native methods across 55 real-world apps, removing over 10K Return-Oriented Programming (ROP) gadgets. Case studies confirm its effectiveness in mitigating vulnerabilities, and performance assessments highlight its resource-saving advantages over non-debloated apps.

==> Comparison.tex <==
%\subsection{Comparison between Dynamic and Static Debloating}
%Before introducing the design of \nameDe, we will compare the similarities and differences between static and dynamic debloating approaches. Existing methods for debloating Android apps offer various ways to identify unneeded code and generate a debloating schema~\cite{jiang_reddroid_2018,xdebloat-tang-2022,liu2024minimon,liu2023autodebloater,thung2024towards}. However, these methods primarily focus on removing unneeded code from the APK file, a process known as static debloating, as it involves statically modifying the APKs before execution. 
%In contrast, the dynamic debloating approach involves installing and running unmodified APKs, then debloating them during runtime by selectively intercepting compilation and execution of target code.

%Table~\ref{tab:comparison} illustrates the comparison between the dynamic debloating approach and static debloating approach across six aspects.
%Specifically, since Android OS originally does not provide the dynamic debloating functionality, we have to modify the Android OS to implement \nameDe. 
%In contrast, static debloating approach only modify the app's APK.
%However, Android mandates that all APKs be digitally signed with a certificate before installation or update~\cite{signWebsite}.
%This signing not only can help identify the developer of an app, but also help protect its integrity.
%Therefore, modifying an APK necessitates resigning it, which nullifies both features.
%Dynamic debloating approach does not for conduct. 
%Besides, although static approaches can debloat DEX or native code, but no existing works are able to debloat them simultaneously from Android apps.
%In contrast, our dynamic debloating approach can debloat code either separately or collectively.
% Static debloating achieves this by removing the DEX or native code from the APK file, while dynamic debloating prevents the DEX code from compiling and the native code from loading into memory.
%Moreover, static debloating makes it challenging to recover debloated code since the code is removed from the APK. Recovering any part of the debloated code requires generating a new APK from the original. In contrast, dynamic debloating facilitates easier recovery of debloated code, as the original APK remains installed, and the code can be recompiled at runtime.
%Similarly, only dynamic debloating allows for changes to the debloating schema at runtime. 
%It can apply a new schema without needing to regenerate and reinstall a new APK.


% Besides, both static and debloating approaches can debloat DEX and native code simultaneously from Android apps, preventing the target executable code (based on the debloating schema) from loading into memory.
% Moreover, static debloating approach cannot easily recover part of the debloated code after the debloating APK is generated, since the debloated code are removed.
% To recover part of the debloated code, they have to generate a new APK from the original APK.
% It is easier for dynamic debloating approach to recover the debloated code, since the original APK is installed, and can be recovered by allowing those code to be compiled during runtime.
